Parameter-Free Style Projection for Arbitrary Style Transfer

Arbitrary image style transfer is a challenging task which aims to stylize a content image conditioned on arbitrary style images. In this task the feature-level content-style transformation plays a vital role for proper fusion of features. Existing feature transformation algorithms often suffer from loss of content or style details, non-natural stroke patterns, and unstable training. To mitigate these issues, this paper proposes a new feature-level style transformation technique, named Style Projection, for parameter-free, fast, and effective content-style transformation. This paper further presents a real-time feed-forward model to leverage Style Projection for arbitrary image style transfer, which includes a regularization term for matching the semantics between input contents and stylized outputs. Extensive qualitative analysis, quantitative evaluation, and user study have demonstrated the effectiveness and efficiency of the proposed methods.

==> fig_ablation.tex <==
\newcommand{\scale}{0.135}

\begin{figure*}[!htb]
\centering
\small

% \includegraphics[width=\scale \linewidth]{figs/ablation/28-scream.jpg}
% \includegraphics[width=\scale \linewidth]{figs/ablation/adain-28_stylized_the_scream.jpg}
% \includegraphics[width=\scale
% \linewidth]{figs/ablation/adain-unet-kl-28_stylized_the_scream.jpg}
% \includegraphics[width=\scale
% \linewidth]{figs/ablation/it-28_stylized_the_scream.jpg}
% \includegraphics[width=\scale \linewidth]{figs/ablation/it-kl-28_stylized_the_scream.jpg}
% %\includegraphics[width=\scale \linewidth]{figs/ablation/it-kl5-28_stylized_the_scream.jpg}
% % \includegraphics[width=\scale  \linewidth]{figs/ablation/it-kl10-28_stylized_the_scream.jpg}
% \includegraphics[width=\scale \linewidth]{figs/ablation/it-unet-28_stylized_the_scream.jpg}
% \includegraphics[width=\scale  \linewidth]{figs/ablation/it-unet-kl-28_stylized_the_scream.jpg}

% \vspace{0.1cm}

\stackunder[5pt]{\includegraphics[width=\scale \linewidth]{figs/ablation/30-feathres.jpg}}{\small Content / Style}
\stackunder[5pt]{\includegraphics[width=\scale \linewidth]{figs/ablation/adain-30_stylized_feathers.jpg}}{\small AdaIN}
\stackunder[5pt]{\includegraphics[width=\scale \linewidth]{figs/ablation/adain-unet-kl-30_stylized_feathers.jpg}}{\small AdaIN+Skip+KL}
\stackunder[5pt]{\includegraphics[width=\scale \linewidth]{figs/ablation/it-30_stylized_feathers.jpg}}{\small SP}
\stackunder[5pt]{\includegraphics[width=\scale \linewidth]{figs/ablation/it-kl-30_stylized_feathers.jpg}}{\small SP+KL}
%\stackunder[5pt]{\includegraphics[width=\scale \linewidth]{figs/ablation/it-kl5-30_stylized_feathers.jpg}}{\small SP+KL($\kappa$=5)}
% \stackunder[5pt]{\includegraphics[width=\scale \linewidth]{figs/ablation/it-kl10-30_stylized_feathers.jpg}}{\small SP+KL($\kappa$=10)}
\stackunder[5pt]{\includegraphics[width=\scale \linewidth]{figs/ablation/it-unet-30_stylized_feathers.jpg}}{\small SP+Skip}
\stackunder[5pt]{\includegraphics[width=\scale \linewidth]{figs/ablation/it-unet-kl-30_stylized_feathers.jpg}}{\small SP+Skip+KL}


\caption{Ablation studies on content skip connections and KL divergence loss. AdaIN can also be benefited from content skip connections and KL divergence loss, showing a more distinct stylized image. }
\label{fig:ablation}
\vspace{0.4em}
\end{figure*}
